Few-shot Image Recognition with Manifolds

In this paper, we extend the traditional few-shot learning (FSL) problem to the situation when the source-domain data is not accessible but only high-level information in the form of class prototypes is available. This limited information setup for the FSL problem deserves much attention due to its implication of privacy-preserving inaccessibility to the source-domain data but it has rarely been addressed before. Because of limited training data, we propose a non-parametric approach to this FSL problem by assuming that all the class prototypes are structurally arranged on a manifold. Accordingly, we estimate the novel-class prototype locations by projecting the few-shot samples onto the average of the subspaces on which the surrounding classes lie. During classification, we again exploit the structural arrangement of the categories by inducing a Markov chain on the graph constructed with the class prototypes. This manifold distance obtained using the Markov chain is expected to produce better results compared to a traditional nearest-neighbor-based Euclidean distance. To evaluate our proposed framework, we have tested it on two image datasets - the large-scale ImageNet and the small-scale but fine-grained CUB-200. We have also studied parameter sensitivity to better understand our framework.

==> header.tex <==
\newcommand{\EQ}{\begin{equation}}
\newcommand{\NQ}{\end{equation}}
\newcommand{\ER}{\begin{eqnarray}}
\newcommand{\NR}{\end{eqnarray}}
\newcommand{\ERS}{\begin{eqnarray*}}
\newcommand{\NRS}{\end{eqnarray*}}
\newcommand{\bit}{\begin{itemize}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\eben}{\end{enumerate}}
\newcommand{\ebit}{\end{itemize}}
\newcommand{\bzero}{{\bf 0}}
\newcommand{\ba}{{\bf a}}
\newcommand{\bb}{{\bf b}}
\newcommand{\bc}{{\bf c}}
\newcommand{\bd}{{\bf d}}
\newcommand{\be}{{\bf e}}
\newcommand{\bbf}{{\bf f}}
\newcommand{\bg}{{\bf g}}
\newcommand{\bh}{{\bf h}}
\newcommand{\bi}{{\bf i}}
\newcommand{\bj}{{\bf j}}
\newcommand{\bk}{{\bf k}}
\newcommand{\bl}{{\bf l}}
\newcommand{\bm}{{\bf m}}
\newcommand{\bn}{{\bf n}}
\newcommand{\bo}{{\bf o}}
\newcommand{\bp}{{\bf p}}
\newcommand{\bq}{{\bf q}}
\newcommand{\br}{{\bf r}}
\newcommand{\bs}{{\bf s}}
\newcommand{\bt}{{\bf t}}
\newcommand{\bu}{{\bf u}}
\newcommand{\bv}{{\bf v}}
\newcommand{\bw}{{\bf w}}
\newcommand{\bx}{{\bf x}}
\newcommand{\by}{{\bf y}}
\newcommand{\bz}{{\bf z}}
\newcommand{\bA}{{\bf A}}
\newcommand{\bB}{{\bf B}}
\newcommand{\bC}{{\bf C}}
\newcommand{\bD}{{\bf D}}
\newcommand{\bE}{{\bf E}}
\newcommand{\bF}{{\bf F}}
\newcommand{\bG}{{\bf G}}
\newcommand{\bH}{{\bf H}}
\newcommand{\bI}{{\bf I}}
\newcommand{\bJ}{{\bf J}}
\newcommand{\bK}{{\bf K}}
\newcommand{\bL}{{\bf L}}
\newcommand{\bM}{{\bf M}}
\newcommand{\bN}{{\bf N}}
\newcommand{\bO}{{\bf O}}
\newcommand{\bP}{{\bf P}}
\newcommand{\bQ}{{\bf Q}}
\newcommand{\bR}{{\bf R}}
\newcommand{\bS}{{\bf S}}
\newcommand{\bT}{{\bf T}}
\newcommand{\bU}{{\bf U}}
\newcommand{\bV}{{\bf V}}
\newcommand{\bW}{{\bf W}}
\newcommand{\bX}{{\bf X}}
\newcommand{\bY}{{\bf Y}}
\newcommand{\bZ}{{\bf Z}}
%\newcommand{\bx}{{\mbox{\boldmath $x$}}}
\newcommand{\balpha}{{\mbox{\boldmath $\alpha$}}}
\newcommand{\blambda}{{\mbox{\boldmath $\lambda$}}}
\newcommand{\bdelta}{{\mbox{\boldmath $\delta$}}}
\newcommand{\boldeta}{{\mbox{\boldmath $\eta$}}}
\newcommand{\bbeta}{{\mbox{\boldmath $\beta$}}}
\newcommand{\bomega}{{\mbox{\boldmath $\omega$}}}
\newcommand{\btau}{{\mbox{\boldmath $\tau$}}}
\newcommand{\ddbtheta}{{\mbox{\boldmath $\ddot{\theta}$}}}
\newcommand{\dbtheta}{{\mbox{\boldmath $\dot{\theta}$}}}
\newcommand{\dbOmega}{{\mbox{\boldmath $\dot{\Omega}$}}}
\newcommand{\dbPhi}{{\mbox{\boldmath $\dot{\Phi}$}}}
\newcommand{\dbomega}{{\mbox{\boldmath $\dot{\omega}$}}}
\newcommand{\btheta}{{\mbox{\boldmath $\theta$}}}
\newcommand{\bzeta}{{\mbox{\boldmath $\zeta$}}}
\newcommand{\bchi}{{\mbox{\boldmath $\chi$}}}
\newcommand{\bmu}{{\mbox{\boldmath $\mu$}}}
\newcommand{\bepsilon}{\hbox{\boldmath{$\epsilon$}}}
\newcommand{\bpi}{\hbox{\boldmath{$\pi$}}}
\newcommand{\brho}{{\mbox{\boldmath $\rho$}}}
\newcommand{\hx}{\hat{x}}
\newcommand{\hq}{\hat{q}}
\newcommand{\bGamma}{{\mbox{\boldmath $\Gamma$}}}
\newcommand{\bOmega}{{\mbox{\boldmath $\Omega$}}}
\newcommand{\bTheta}{{\mbox{\boldmath $\Theta$}}}
\newcommand{\bSigma}{{\mbox{\boldmath $\Sigma$}}}
\newcommand{\bDelta}{{\mbox{\boldmath $\Delta$}}}
\newcommand{\bPhi}{{\mbox{\boldmath $\Phi$}}}
\newcommand{\domega}{{\mbox{$\dot{\omega}$}}}
\newcommand{\dPhi}{{\mbox{$\dot{\Phi}$}}}
\newcommand{\dzeta}{{\mbox{$\dot{\zeta}$}}}
\newcommand{\dbeta}{{\mbox{$\dot{\beta}$}}}
\newcommand{\dalpha}{{\mbox{$\dot{\alpha}$}}}
\newcommand{\dgamma}{{\mbox{$\dot{\gamma}$}}}
\newcommand{\hbx}{{\bf \hat{x}}}
\newcommand{\hby}{{\bf \hat{y}}}
\newcommand{\hbq}{{\bf \hat{q}}}
\newcommand{\ddbe}{{\bf \ddot e}}
\newcommand{\ddbv}{{\bf \ddot v}}
\newcommand{\ddbp}{{\bf \ddot p}}
\newcommand{\ddbq}{{\bf \ddot q}}
\newcommand{\ddbx}{{\bf \ddot x}}
\newcommand{\ddby}{{\bf \ddot y}}
\newcommand{\dbe}{{\bf \dot e}}
\newcommand{\dbh}{{\bf \dot h}}
\newcommand{\dbp}{{\bf \dot p}}
\newcommand{\dbr}{{\bf \dot r}}
\newcommand{\dbx}{{\bf \dot x}}
\newcommand{\dby}{{\bf \dot y}}
\newcommand{\dbu}{{\bf \dot u}}
\newcommand{\dbv}{{\bf \dot v}}
\newcommand{\dbq}{{\bf \dot q}}
\newcommand{\dbJ}{{\bf \dot J}}
\newcommand{\dbN}{{\bf \dot N}}
\newcommand{\dbA}{{\bf \dot A}}
\newcommand{\dE}{\dot E}
\newcommand{\dL}{\dot L}
\newcommand{\de}{\dot e}
\newcommand{\ds}{\dot s}
\newcommand{\dw}{\dot w}
\newcommand{\dq}{\dot q}
\newcommand{\dx}{\dot x}
\newcommand{\dy}{\dot y}
\newcommand{\dz}{\dot z}
\newcommand{\dde}{\ddot e}
\newcommand{\ddx}{\ddot x}
\newcommand{\ddy}{\ddot y}
\newcommand{\ddz}{\ddot z}
\newcommand{\ddq}{\ddot q}
\newcommand{\dtheta}{\dot \theta}
\newcommand{\ddtheta}{\ddot \theta}
%\newcommand{\dbomega}{{\bf \dot \omega}}
%\newcommand{\mdot}{{\scriptscriptstyle\bullet}}
%\newcommand{\mdot}{\mbox{\boldmath $\cdot$}}
\newcommand{\defn}{\buildrel \rm \triangle \over =}
\newcommand{\anddot}{\buildrel \wedge \over \cdot}
\newcommand{\ordot}{\buildrel \codt \over \vee}
\newcommand{\prob}{\hbox{prob}}
\newcommand{\prop}{\hbox{prop}}
\newcommand{\ttan}{\hbox{atan2}}
\newcommand{\usually}{\hbox{usually}}
\newcommand{\Tr}{\hbox{ Tr}}
\newcommand{\rand}{\hbox{ and }}
\newcommand{\are}{\hbox{ are }}
\newcommand{\ror}{\hbox{ or }}
\newcommand{\is}{\hbox{ is }}
\newcommand{\ie}{\hbox{i.e.,}}
\newcommand{\poss}{\hbox{poss}}
\newcommand{\CON}{\hbox{CON}}
\newcommand{\DIL}{\hbox{DIL}}
\newcommand{\INT}{\hbox{INT}}
\newcommand{\sgn}{\hbox{sgn}}
\newcommand{\net}{\hbox{net}}
%\newcommand{\block}{\rule{2mm}{2mm}}
\newcommand{\ralpha}{\stackrel{\alpha}{\leftrightarrow}}
\newcommand{\cf}{\stackrel{cf}{\rightarrow}}
\newcommand{\one}{\stackrel{1}{\rightarrow}}
\newcommand{\gef}{\buildrel > \over =}
\newcommand{\lef}{\buildrel < \over =}
\newcommand{\half}{{1 \over 2}}
\newcommand{\dst}{\everymath{\displaystyle}} %---- use displaystle in eqs.
\newcommand{\Nuclide}[2]{${}^{#2}$#1}        %---- Nuclide macro
%\newcommand{\SS}[1]{${}^{#1}$}               %---- superscript in text
\newcommand{\STRUT}{\rule{0in}{3ex}}         %--- small strut
\newcommand{\dotprod}{{\scriptscriptstyle \stackrel{\bullet}{{}}}}
\newcommand{\bFR}{\mit{FR}}

\newenvironment{emphasis}[1]{\begin{quote}{\bf #1\/}:}{\end{quote}}

\newcommand{\namelistlabel}[1]{\mbox{#1}\hfill }
\newenvironment{namelist}[1]{%
\begin{list}{}
{
  \let\makelabel\namelistlabel
  \settowidth{\labelwidth}{#1}
  \setlength{\leftmargin}{1.1\labelwidth}
}
}{%
\end{list}}

\def\m@th{\mathsurround=0pt }

\def\eqalign#1{\null\,\vcenter{\openup1\jot \m@th
  \ialign{\strut\hfil$\displaystyle{##}$&$\displaystyle{{}##}$\hfil
      \crcr#1\crcr}}\,}


%\evensidemargin=-0.3in

%Letter Size: 8.5 X 11 in
%\textwidth=6.5truein
%\textheight=8.8truein

%A4 Size
%\textwidth=6.8truein
%\textheight=9.3truein

\def\doublespace{
   \global\baselineskip=24truept plus 4truept%
   \lineskip=10truept%
   \lineskiplimit=10truept%
   \parskip=10truept
}%doublespace

\def\onehalfspace{
%   \global\baselineskip=18truept plus 3truept%
   \global\baselineskip=16truept plus 3truept%
   \lineskip=7.5truept%
   \lineskiplimit=7.5truept%
   \parskip=10truept
}%onehalfspace

\def\singlespace{
   \global\baselineskip=12truept plus 1truept%
   \lineskip=3truept%
   \lineskiplimit=3truept%
   \parskip=6truept
}%singlespace

%\def\singlespace{
%   \global\baselineskip=9truept plus 1truept%
%   \lineskip=3truept%
%   \lineskiplimit=3truept%
%   \parskip=5truept
%}%singlespace

%\def\normalbaselines{\lineskip=\normalineskip
%   \baselineskip=\normalbaselineskip \lineskiplimit=\normallineskiplimit}

%\def\openup{\afterassignment\@penup\dimen@=}
%\def\@penup{\advance\lineskip\dimen@
%  \advance\baselineskip\dimen@ \advance\lineskiplimit\dimen@}


%\newif\ifdt@p
\def\displ@y{\global\dt@ptrue \openup1\jot \m@th
  \everycr{\noalign{\ifdt@p \global\dt@pfalse
      \vskip-\lineskiplimit \vskip\normallineskiplimit
      \else \penalty\interdisplaylinepenalty \fi}}}
%\def\displ@y{\dt@ptrue \openup1\jot \m@th
%  \everycr{\noalign{\ifdt@p \dt@pfalse
%      \vskip-\lineskiplimit \vskip\normallineskiplimit
%      \else \penalty\interdisplaylinepenalty \fi}}}
\def\@lign{\tabskip=0pt\everycr={}} % restore inside \displ@y
%\def\displaylines#1{\displ@y
%  \halign{\hbox to\displaywidth{$\hfil\@lign\displaystyle##\hfil$}\crcr
%    #1\crcr}}

\def\eqalignno#1{\displ@y \tabskip=\centering
  \halign to\displaywidth{\hfil$\@lign\displaystyle{##}$\tabskip=0pt
    &$\@lign\displaystyle{{}##}$\hfil\tabskip=\centering
    &\llap{$\@lign##$}\tabskip=0pt\crcr
    #1\crcr}}

\def\oalpha{{\ooalign{\hfil\raise.07ex\hbox{$\alpha$}\hfil\crcr\mathhexbox20D}}}
%\def\obeta{{\ooalign{\hfil\raise.07ex\hbox{$\beta$}\hfil\crcr\mathhexbox20D}}}
%\def\ot{{\ooalign{\hfil\raise.07ex\hbox{$t$}\hfil\crcr\mathhexbox20D}}}

\def\ooalpha{{\ooalign{\hfil\raise.07ex\hbox{$\alpha$}\hfil\crcr$\textstyle{\circ}t$}}}

\def\obeta{{\ooalign{\hfil\raise.07ex\hbox{$\scriptstyle{\beta}$}\hfil\crcr$\textstyle{\circ}$}}}

\def\ot{{\ooalign{\hfil\raise.07ex\hbox{$t$}\hfil\crcr$\textstyle{\circ}$}}}

\def\oooalpha{{\ooalign{\hfil\raise.07ex\hbox{${\scriptstyle{\alpha}}$}\hfil\crcr${\textstyle{\circ}}$}}}

%\def\oooalpha{{\ooalign{\hfil\raise.07ex\hbox{${\scriptstyle{\alpha}}$}\hfil\crcr${\scriptscriptstyle{\mathhexbox20D}$}}}}

%\def\leqalignno#1\displ@y \tabskip=\centering
%  \halign to\displaywidth{\hfil$\@lign\displaystyle{##}$\tabskip=0pt
%    &$\@lign\displaystyle{{}##}$\hfil\tabskip=\centering
%    &\kern-\displaywidth\rlap{$\@lign##$}\tabskip=\displaywidth\crcr
%    #1\crcr}}


%\def\trade{{\oalign#1{\leavevmode\vtop{\baselineskip\z@skip \lineskip.25ex%
%  \ialign{##\crcr#1\crcr}}}}} % put characters over each other
%\def\ooalign{\lineskiplimit-\maxdimen \oalign}
%\def\d#1{\oalign{#1\crcr\hidewidth.\hidewidth}}
%\def\b#1{\oalign{#1\crcr\hidewidth
%    \vbox to.2ex{\hbox{\char22}\vss}\hidewidth}}
%\def\c#1{\setbox\z@\hbox{#1}\ifdim\ht\z@=1ex\accent24 #1%
%  \else{\ooalign{\hidewidth\char24\hidewidth\crcr\unhbox\z@}}\fi}
\def\trademark{{\ooalign{\hfil\raise.07ex\hbox{R}\hfil\crcr\mathhexbox20D}}}

